Multi-Stage Active Sequential Hypothesis Testing with Clustered Hypotheses

We consider the problem where an active Decision-Maker (DM) is tasked to identify the true hypothesis using as few as possible observations while maintaining accuracy. The DM collects observations according to its determined actions and knows the distributions under each hypothesis. We propose a deterministic and adaptive multi-stage hypothesis-elimination strategy where the DM selects an action, applies it repeatedly, and discards hypotheses in light of its obtained observations. The DM selects actions based on maximal separation expressed by the distance between the parameter vectors of each distribution under each hypothesis. Close distributions can be clustered, simplifying the search and significantly reducing the number of required observations. Our algorithms achieve vanishing Average Bayes Risk (ABR) as the error probability approaches zero, i.e., the algorithm is asymptotically optimal. Furthermore, we show that the ABR is bounded when the number of hypotheses grows. Simulations are carried out to evaluate the algorithm's performance compared to another multi-stage hypothesis-elimination algorithm, where an improvement of several orders of magnitude in the mean number of observations required is observed.

==> 01_ISIT25v2/TeXFiles/Numerical_Results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical Results}
\label{subsection: Numerical Results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we present numerical results illustrating the performance of our algorithm compared to GJL.
To this end, we have conducted simulations.
In the simulations, we have used uniform priors, i.e., $\pi_i = \frac{1}{H}$.
For a fair comparison, we have picked distributions whose mean estimation can distinguish between different hypotheses, namely, the exponential and unit-variance normal distributions.
Accordingly, observations obtained by each action differ in their mean.

The number of hypotheses was set to $H=4$, and the \ac{DM} had $\abs{\mathcal{A}} = H+1 = 5$ actions.
The first $H$ actions had a mean of 3 if $H_{a-1}$ is true for $1\leq a\leq 4$, and a random mean drawn uniformly from $[0, 1]$ otherwise.
The last action, designed to be selected by the greedy algorithm, had the means follow the equation $0.5 + 0.01\times i$ for $0\leq i\leq 4$.
All random parameters were drawn only once at the beginning of the simulation.

For the clustering algorithm, DBSCAN, we use $\text{minPts}=1$ and proximity parameters $\varepsilon\in\{0, 0.3, 1\}$.
Namely, we compare GJL to our algorithm in three scenarios: (i) when no clustering is used ($\varepsilon=0$). (ii) when selecting a suitable proximity parameter ($\varepsilon=0.3$). (iii) when the proximity parameter is too large ($\varepsilon=1$).
Note that $\varepsilon = 1$ is too large since points are clustered into at most two clusters regardless of the drawn numbers, and more importantly, it may violate the requirement that \eqref{eq: AEP res} is positive.

In Figure \ref{figure: avg Bayes Risk vs. delta eps}, we present the results for a scenario when all actions produce observations following the normal distribution.
With the exception of the poor choice of $\varepsilon=1$, each algorithm attains vanishing \ac{ABR} as $\delta\to 0$, but the non-greedy selections made by our algorithm enjoy a faster decay.
We attribute the decay to the number of observations needed until declaration.
To properly connect them, we approximate the error probability $p_e$ to $\delta$ to observe that
\begin{align}
    \nonumber
    \frac{\delta}{H^2}\expVal{N} + p_e
    \approx
    \frac{\delta}{H^2}\expVal{N} + \delta
    =
    \delta
    \left(
        \frac{\expVal{N}}{H^2} + 1
    \right)
    .
\end{align}
Hence, the logarithm of the \ac{ABR} (y-axis) decreases linearly in $\log \frac{1}{\delta}$ (x-axis), and its intersection point with the y-axis solely depends on the average number of observations taken.
Therefore, the instances of our algorithm with $\varepsilon\in\{0, 0.3\}$ have lower \ac{ABR} since they require no more observations on average than GJL, which takes a fixed number of observations inversely proportional to the \ac{KLD} between the correct hypothesis and its closest hypothesis (i.e., the worst average case).
We emphasize that when $\varepsilon = 0.3$, our algorithm stopped its hypothesis identification earlier than GJL or the $\varepsilon=0$ instance since the algorithm identified the correct cluster and moved to the next action that can better separate the newly identified cluster. 

\begin{figure}
    \centering
    \ifCompileImages
        \input{01_ISIT25v1/TeXFiles/TeXImages/Average Bayes Risk vs delta eps norm}
        \vspace{-24pt}
    \else
        \includegraphics[]{01_ISIT25v1/Images/Average Bayes Risk vs delta eps norm}
        \vspace{-8pt}
    \fi
    \caption{
        Comparison of the \ac{ABR} for $H = 4$ and $\abs{\mathcal{A}} = 5$ using our algorithm (with proximity parameter $\varepsilon\in\{0, 0.3, 1\}$) against GJL.
        All actions produce normally distributed observations.
        The \ac{ABR} approaches zero as $\delta\to 0$ for all instances, but the greedy selection results in a slower decay.
    }
    \label{figure: avg Bayes Risk vs. delta eps}
\end{figure}

% \begin{table}[!htbp]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%           & $H_0$ & $H_1$ & $H_2$ & $H_3$ \\
%           \hline
%         1 & 3 & 0.7 & 0.825 & 0.311\\
%         2 & 0.001 & 3 & 0.815 & 0.63\\
%         3 & 0.717 & 0.206 & 3 & 0.17\\
%         4 & 0.405 & 0.201 & 0.263 & 3\\
%         5 & 0.5 & 0.51 & 0.52 & 0.53\\
%     \end{tabular}
%     \vspace{3pt}
%     \caption{The means used for Figure \ref{figure: avg Bayes Risk vs. delta eps exp} (up to three digits)}
%     \label{tab: exp means}
% \end{table}

In Figure \ref{figure: avg Bayes Risk vs. delta eps exp}, we repeat the same experiment as the previous one, but each action produces exponentially distributed samples.
Here, the choice of $\varepsilon = 1$ made the \ac{ABR} converge to $\frac{1}{2}$, as the partition into two clusters (mean $3$ and any other parameter) is an inappropriate partition of the distributions.

\begin{figure}
    \centering
    \ifCompileImages
        \input{01_ISIT25v1/TeXFiles/TeXImages/Average Bayes Risk vs delta eps exp}
        \vspace{-24pt}
    \else
        \includegraphics[]{01_ISIT25v1/Images/Average Bayes Risk vs delta eps exp}
        \vspace{-8pt}
    \fi
    \caption{
        Comparison of the \ac{ABR} for $H = 4$ and $\abs{\mathcal{A}} = 5$ using our algorithm (with proximity parameter $\varepsilon\in\{0, 0.3, 1\}$) against GJL.
        All actions produce exponentially distributed observations.
        The \ac{ABR} approaches zero as $\delta\to 0$ for all instances, but the greedy selection results in a slower decay.
        Our algorithm may misbehave when choosing an inappropriate value of $\varepsilon$.
    }
    \label{figure: avg Bayes Risk vs. delta eps exp}
\end{figure}


% \begin{figure}[!htbp]
%     \centering
%     \ifCompileImages
%         \input{01_ISIT25v1/TeXFiles/TeXImages/ABR vs delta (merged)}
%         \vspace{-24pt}
%     \else
%         \includegraphics[]{01_ISIT25v1/Images/ABR vs delta (merged)}
%         \vspace{-8pt}
%     \fi
%     \caption{
%         Comparison of the \ac{ABR} for $H = 4$ and $\abs{\mathcal{A}} = 5$ using our algorithm (with proximity parameter $\varepsilon\in\{0, 0.3, 1\}$) against GJL.
%         All actions produce exponentially distributed observations.
%         The \ac{ABR} approaches zero as $\delta\to 0$ for all instances, but the greedy selection results in a slower decay.
%         Our algorithm may misbehave when choosing an inappropriate value of $\varepsilon$.
%     }
%     \label{figure: avg Bayes Risk vs. delta eps exp norm merged}
% \end{figure}



==> Math_Shortcuts.tex <==
%% Math mode only
\newcommandx{\myVec}[2][2=]{{\underline{#1}_{#2}}}                              %  Defines how vectors look like
\newcommandx{\myMat}[2][2=]{{\mathbf{#1}_{#2}}}                                 %  Defines how matrices look like
\newcommandx{\vectorComponent}[4][3=, 4=]{{[\myVec{#1}_{#3}]_{#2}^{#4}}}        %  Defines how a component of a vector looks like
\newcommandx{\matrixComponent}[4][4=]{{[\myMat{#1}_{#4}]_{#2,#3}}}              %  Defines how a component of a matrix looks like
\newenvironment{lbmatrix}[1]
    {\left(\array{@{}*{#1}c@{}}}
    {\endarray\right)}                                                          %  New matrix format (allows pretty \hlines)
\newcommand{\KLD}[2]{\mathcal{D}_{KL} ( #1 \Vert #2 )}                          %  Kullback-Leibler Divergence
\newcommand{\DKLD}[4]{\Delta\mathcal{D}_{#2#3|#1}(#4)}
\newcommand{\DKLDnoA}[3]{\Delta\mathcal{D}_{#2#3|#1}}
\newcommand{\DKLDdefault}[0]{\DKLDnoA{i}{j}{k}}
\newcommand{\DKLDdefaultA}[0]{\DKLD{i}{j}{k}{a}}
\newcommand{\MI}[2]{I\left( #1 ; #2\right)}                                     %  Mutual Information
\newcommand{\intSet}[2]{[#1, #2]}                                               %  Integer set
\newcommandx{\expVal}[2][2=]{\mathbb{E}_{#2}\left[#1\right]}                    %  Expected value
\newcommand{\indicator}[1]{ \mathds{1}{\left\{#1\right\}} }                     %  Indicator
\newcommand{\prob}[1]{\operatorname{\mathbb{P}}\left( #1 \right)}               %  Probability
\newcommand{\bigO}[1]{\operatorname{\mathcal{O}}\left( #1 \right)}               %  Big-O
\newcommand{\hII}{H_i}
\newcommand{\hJJ}{H_j}
\newcommand{\hKK}{H_k}
\newcommand{\hAlive}{H_{\mathrm{alive}}}
\newcommand{\argmax}[2]{\mathop{\operatorname{argmax}}_{#2} \left\{#1\right\}}
\newcommand{\argmin}[2]{\mathop{\operatorname{argmin}}_{#2} \left\{#1\right\}}
\newcommand{\abs}[1]{ | #1 |}
\newcommand{\equivIndex}[2]{\operatorname{equiv}\left( #1, #2 \right)}
\newcommand{\paramSet}[1]{\operatorname{param}\left( #1 \right)}
\newcommand{\neighborhood}[2]{ \mathcal{B}_{#2} ( #1 ) }
\newcommand{\repr}[2]{\operatorname{repr}\left( #1, #2 \right)}
\newcommand{\ceil}[1]{\left\lceil {#1} \right\rceil}
\newcommand{\floor}[1]{\left\lfloor {#1} \right\rfloor}
\newcommandx{\norm}[2][2=2]{\| #1 \|_{#2}}
\newcommand{\indexedSet}[3]{\myVec{#1}_{#2}^{#3}}


